Fill in the Blank: Exploring and Enhancing LLM Capabilities for Backward Reasoning in Math Word Problems

While forward reasoning (i.e., find the answer given the question) has been explored extensively in recent literature, backward reasoning is relatively unexplored. We examine the backward reasoning capabilities of LLMs on Math Word Problems (MWPs): given a mathematical question and its answer, with some details omitted from the question, can LLMs effectively retrieve the missing information? On modifying three benchmark datasets for this task, to evaluate this task: GSM8k, SVAMP, and MultiArith, we find a significant drop in the accuracy of models on this task compared to forward reasoning across SOTA LLMs (GPT4, GPT3.5, PaLM-2, and LLaMa). Motivated by the fact backward reasoning can be seen as the ''inverse'' of forward reasoning, we propose variations of three different forward reasoning strategies to improve performance. Rephrase reformulates the given problem into a forward reasoning problem, PAL-Tools combines the idea of Program-Aided LLMs to produce a set of equations that can be solved by an external solver, and Check your Work exploits the availability of natural verifier of high accuracy in the forward direction, interleaving solving and verification steps. Finally, realizing that each of our base methods correctly solves a different set of problems, we propose a novel Bayesian formulation for creating an ensemble over the base methods to further boost the accuracy. Extensive experimentation demonstrates successive improvement in the performance of LLMs on the backward reasoning task, using our strategies, with our ensemble-based method resulting in significant performance gains compared to the SOTA forward reasoning strategies we adapt.

==> sections/E00-Intersection.tex <==
\section{Comparative Analysis of Forward and Backward Reasoning Problems}
\label{sec:interesction}
As a preliminary analysis, we counted the number of questions that an LLM was able to solve exclusively for the forward task, exclusively for the backward task, and for both. As observed in table \ref{tab:fw_bw_interesection}, nearly all the questions that the LLM can solve for the backward task are a subset of those it can solve for the forward task. It is important to note, as discussed in Section \ref{sec:other-analysis}, that not all backward task solutions need the forward task's answer, making it a comparatively easier problem to solve.
\begin{table}[H]
  \fontsize{9}{11}\selectfont
  \centering
 %\captionsetup{labelformat=empty}
        
      \begin{tabular}{lrrr}
        \toprule
         & \multicolumn{3}{c}{Task} \\ \cmidrule(lll){2-4} 
         Model & forward only & backward only & both tasks\\
        \midrule
        GPT-4  & 55.50 & 1.34 & 37.26 \\
    %   GPT-3.5 & 45.75 & 5.58 & 12.66 \\
        PaLM-2  & 51.1 & 5.82  & 9.35\\
        LLaMa-2-70B & 32.00 & 3.22 & 3.62 \\
        \bottomrule
      \end{tabular}
\caption{Percentage of problems of GSM8k solved for only the forward task, backward task, and both}
    \label{tab:fw_bw_interesection}
\end{table}


%or we can write 3.47% of correct backward have incorrect forward, rest correct - GPT-4
% 35.25% for PALM-2
% 47.35% for LLaMa
%or we can make Venn Diagrams
